The Benefits of Being Distributional: Small-Loss Bounds for Reinforcement Learning

While distributional reinforcement learning (DistRL) has been empirically effective, the question of when and why it is better than vanilla, non-distributional RL has remained unanswered. This paper explains the benefits of DistRL through the lens of small-loss bounds, which are instance-dependent bounds that scale with optimal achievable cost. Particularly, our bounds converge much faster than those from non-distributional approaches if the optimal cost is small. As warmup, we propose a distributional contextual bandit (DistCB) algorithm, which we show enjoys small-loss regret bounds and empirically outperforms the state-of-the-art on three real-world tasks. In online RL, we propose a DistRL algorithm that constructs confidence sets using maximum likelihood estimation. We prove that our algorithm enjoys novel small-loss PAC bounds in low-rank MDPs. As part of our analysis, we introduce the $\ell_1$ distributional eluder dimension which may be of independent interest. Then, in offline RL, we show that pessimistic DistRL enjoys small-loss PAC bounds that are novel to the offline setting and are more robust to bad single-policy coverage.

==> rwstyle.tex <==
\RequirePackage{nicefrac}
\RequirePackage{amsfonts}
\RequirePackage{dsfont}
\RequirePackage{setspace}

\def\*#1{\bm{#1}} 
\def\+#1{\mathcal{#1}}
\def\=#1{\mathbb{#1}}
\def\##1{\mathfrak{#1}}
\def\^#1{\hat{#1}} 
\def\-#1{\overline{#1}}
\def\~#1{\tilde{#1}}
\def\@#1{{\rm{#1}}}
\def\w~#1{\widetilde{#1}}

\def\indic{\mathds{1}}
\def\d{\mathop{}\!\mathrm{d}}
\def\E{\mathop{\mathbb{E}}}
\def\KL{D_{\rm{KL}}}
\def\argmax{\mathop{\arg\max}}
\def\argmin{\mathop{\arg\min}}
\def\given{\,|\,}

\newcommand\red[1]{\textcolor{red}{#1}}
\newcommand\blue[1]{\textcolor{blue}{#1}}
\newcommand\purple[1]{\textcolor{purple}{#1}}
\newcommand\orange[1]{\textcolor{orange}{#1}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
